A Positive/Unlabeled Approach for the Segmentation of Medical Sequences using Point-Wise Supervision

The ability to quickly annotate medical imaging data plays a critical role in training deep learning frameworks for segmentation. Doing so for image volumes or video sequences is even more pressing as annotating these is particularly burdensome. To alleviate this problem, this work proposes a new method to efficiently segment medical imaging volumes or videos using point-wise annotations only. This allows annotations to be collected extremely quickly and remains applicable to numerous segmentation tasks. Our approach trains a deep learning model using an appropriate Positive/Unlabeled objective function using sparse point-wise annotations. While most methods of this kind assume that the proportion of positive samples in the data is known a-priori, we introduce a novel self-supervised method to estimate this prior efficiently by combining a Bayesian estimation framework and new stopping criteria. Our method iteratively estimates appropriate class priors and yields high segmentation quality for a variety of object types and imaging modalities. In addition, by leveraging a spatio-temporal tracking framework, we regularize our predictions by leveraging the complete data volume. We show experimentally that our approach outperforms state-of-the-art methods tailored to the same problem.

==> tables/mae.tex <==
\begin{table}
\centering
\label{tab:mae}
\caption{Mean Absolute Error and standard deviation of estimated class-priors for all types for different initial conditions.}
\begin{tabular}{p{1.8cm}p{1.8cm}p{1.8cm}}
\toprule
piovrs &                   1.4 &                   1.6 \\
Types    &                       &                       \\
\midrule
Brain    &    $\bm{0.0} \pm nan$ &       $0.01 \pm 0.01$ \\
Cochlea  &  $\bm{0.02} \pm 0.01$ &       $0.04 \pm 0.04$ \\
Slitlamp &   $\bm{0.01} \pm nan$ &        $0.01 \pm 0.0$ \\
Tweezer  &       $0.02 \pm 0.03$ &  $\bm{0.01} \pm 0.01$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/pu_vs_true.tex <==
\begin{table*}[t]
\centering
\caption{
Quantitative results on all datasets. We report the F1 scores and standard deviations.
}
\label{tab:results}
\begin{tabular}{llp{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}}
\toprule
Types &                 Brain &               Cochlea &              Slitlamp &               Tweezer \\
Methods            &                       &                       &                       &                       \\
\midrule
KSPTrack/nnPUtrue      &       $\bm{0.84} \pm 0.05$ &  $\bm{0.75} \pm 0.04$ &  $\bm{0.88} \pm 0.02$ &       $\bm{0.93} \pm 0.01$ \\
KSPTrack/aaPUtrees &       $0.77 \pm 0.12$ &       $0.68 \pm 0.08$ &       $0.84 \pm 0.05$ &       $0.92 \pm 0.01$ \\
KSPTrack/aaPU      &  $0.81 \pm 0.08$ &       $0.62 \pm 0.13$ &       $0.84 \pm 0.06$ &  $0.92 \pm 0.01$ \\
KSPTrack/nnPU      &       $0.76 \pm 0.11$ &  $0.69 \pm 0.07$ &  $0.85 \pm 0.05$ &       $0.91 \pm 0.01$ \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/results_tmp.tex <==
\begin{table*}[t]
\centering
\caption{
    Quantitative results on all datasets. We report the F1 scores and standard deviations.
    }
\label{tab:results}
\begin{tabular}{llp{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}}
\toprule
Types &                 Brain &               Cochlea &              Slitlamp &              Tweezer \\
Methods       &                       &                       &                       &                      \\
\midrule
Truth         &       $0.92 \pm 0.02$ &       $0.92 \pm 0.01$ &       $0.92 \pm 0.02$ &      $0.95 \pm 0.01$ \\
\hline

KSPTrack/nnPU &                  0.74 &                  0.66 &                  0.73 &  $\bm{0.9} \pm 0.02$ \\
nnPU          &                   0.7 &                  0.45 &  $\bm{0.82} \pm 0.02$ &                 0.76 \\
\hdashline
KSPTrack      &  $\bm{0.74} \pm 0.08$ &  $\bm{0.66} \pm 0.02$ &                  0.77 &                 0.77 \\
EEL           &                  0.52 &                  0.12 &                  0.59 &                  0.6 \\
Gaze2Segment  &                  0.07 &                  0.07 &                  0.02 &                 0.18 \\
DL-prior      &                  0.56 &                   0.3 &                  0.51 &                 0.72 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/results_vs_true.tex <==
\begin{table*}[t]
\centering
\caption{
    Quantitative results on all datasets of proposed method with true class-priors. We report the F1 scores and standard deviations.
    }
\label{tab:results_vs_true}
\begin{tabular}{llp{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}}
\toprule
Types &                Brain &               Cochlea &              Slitlamp &               Tweezer \\
Methods           &                      &                       &                       &                       \\
\midrule
KSPTrack/nnPUtrue &  $\bm{0.8} \pm 0.09$ &  $\bm{0.78} \pm 0.05$ &  $\bm{0.86} \pm 0.03$ &       $\bm{0.92} \pm 0.02$ \\
KSPTrack/nnPU     &       $0.79 \pm 0.1$ &       $0.69 \pm 0.03$ &       $0.85 \pm 0.05$ &  $0.91 \pm 0.03$ \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/sp_errors.tex <==
\begin{table}
\centering
\caption{For each type of sequence, we report the maximum F1-score achievable given the early stage superpixel segmentation.}
\label{tab:sp_errors}
\begin{tabular}{lp{1.8cm}}
\toprule
{} &               F1 \\
\midrule
Brain    &  $0.92 \pm 0.02$ \\
Cochlea  &  $0.92 \pm 0.01$ \\
Slitlamp &  $0.92 \pm 0.02$ \\
Tweezer  &  $0.95 \pm 0.01$ \\
\bottomrule
\end{tabular}
\end{table}

